Frequency learning for image classification

Machine learning applied to computer vision and signal processing is achieving results comparable to the human brain on specific tasks due to the great improvements brought by the deep neural networks (DNN). The majority of state-of-the-art architectures nowadays are DNN related, but only a few explore the frequency domain to extract useful information and improve the results, like in the image processing field. In this context, this paper presents a new approach for exploring the Fourier transform of the input images, which is composed of trainable frequency filters that boost discriminative components in the spectrum. Additionally, we propose a slicing procedure to allow the network to learn both global and local features from the frequency-domain representations of the image blocks. The proposed method proved to be competitive with respect to well-known DNN architectures in the selected experiments, with the advantage of being a simpler and lightweight model. This work also raises the discussion on how the state-of-the-art DNNs architectures can exploit not only spatial features, but also the frequency, in order to improve its performance when solving real world problems.

==> source/1_intro.tex <==
% !TeX encoding = UTF-8
% !TeX spellcheck = en_US

\IEEEraisesectionheading{\section{Introduction}\label{sec:introduction}}
\label{sec:intro}

% general introduction

Machine learning (ML) have changed many applications in the last years, especially in computer vision and signal processing areas\cite{goodfellow2016deep}. The number of applications based on deep learning are exploding and giving to the computer more reliability to solve complex problems such as aiding medical diagnosis and autonomously driving cars. The human brain is the main inspiration for these systems, since it has a noticeable ability to solve problems in a parallel and complex way\cite{haykin2009neural}.

% RNA introduction

The brain has a plasticity that enables the nervous system to adapt according to the environment in which it is inserted. This plasticity enables the neurons to process data and extract useful information. In the same way, artificial neural networks (ANNs) process data and learn from it. 

%The ANNs have artificial neurons in their architectures, which have an adaptive structure (or plasticity) which can learn from the presented data~\cite{haykin2009neural}. Each neuron has a simple structure that allows it to learn a simple function but when connected with other neurons, in a massive way, it is possible to learn more complex models due the amount of connections between them. %
The neuron model, how they are connected and how they learn basically define the network architecture. Based on this architecture, the ANN can learn from data and store experimental knowledge, making it available for further applications\cite{haykin2009neural}.

% DNN intro
The progress of learning algorithms, the availability of large datasets and the possibility of using highly parallel hardware, with graphic processing units (GPU), greatly boosted the success of ANN applications in the last decade. 
In this scenario, deep and more complexes architectures started to be used to solve difficult problems in many different fields, being the state-of-the-art in many areas, such as speech and text processing, and computer vision\cite{lecun2015deep}. 

% SUBSTITUIDO PELO ABAIXO --> When working with data, traditional machine learning techniques do not perform well when processing them as they are capture (raw data). In this case, to build a pattern recognition application, for example, it is necessary to transform the raw data in proper features, normally in a reduced dimensional. This requires a high domain knowledge specialist to design the proper extractor that will provide discriminative features, allowing the classifier to learn from them and correct recognize different input patterns\cite{lecun2015deep}. Examples of these handcrafted features are \textit{Mel-frequency cepstral coefficients (MFCC)}\cite{davis1980comparison}  for sound processing, and \textit{speeded up robust features (SURF)}\cite{bay2006surf} for image processing. Both demanded long time and a high specialized human team to design them.
Traditionally, the effective use of machine learning techniques involved a preprocessing stage, in which the available raw data was transformed into proper features, usually with a reduced dimensionality when compared to the original data. This approach requires a careful design of the feature extractor by experts with high domain knowledge, in order that discriminative features are attained and, ultimately, the ML model reaches an adequate performance. Some well-known examples of handcrafted features are the mel-frequency cepstral coefficients (MFCC)\cite{davis1980comparison} for sound processing, and speeded up robust features (SURF)\cite{bay2006surf} for image processing. Both techniques demanded a long time and a highly specialized research team to be developed. 


% SUBSTITUIDO PELO ABAIXO --> On the other hand, when working with deep learning, these features can be learned directly from the data. The challenge here is to develop the proper architecture to solve that specific problem. In a computer vision application, for example, the model will learn directly from the image pixels. Consider a basic example in the face recognition scenario: first layers of the network will extract more simple features, such as borders and corners; the next layers will use these features to form small blocks from the face, like circles, rectangles and triangles; the layer in the sequence will use these features from the previous layers to create more complexes shapes such as nose, ear, mouth and so on. Based on this aggregated information extracted from the layers, system will be able to perform the classification and distinguish different faces. In this sense, the features are not designed by a human expert, but learned directly from the data \cite{lecun2015deep}. Different features can be learned for different problems. For example, the extractors learned for car recognition will be different from that ones learned for fruit recognition. This make the network more flexible according to the problem that needs to be solved, improving results in the majority of the cases when compared to generic handcrafted features.

On the other hand, the approach explored in deep learning is to let the model learn directly from the raw data. In this sense, the deep model indirectly creates efficient internal representations for the data while it is learning how to perform the desired task (e.g., to classify images). Additionally, the deep and layered structure of the model gives rise to a hierarchical representation, since the first layers tend to extract low level features, which are progressively combined into high level features by the subsequent layers. Given the high flexibility of the deep models, this perspective proved to be advantageous in several challenging real-world tasks, leading to superior results when compared with using generic handcrafted features. 
Among the most prominent deep models, the convolutional neural networks (ConvNets)\cite{goodfellow2016deep} stand out in the field of computer vision, especially after 2012\cite{krizhevsky2012imagenet}. 

%Considering this, many deep architectures have been proposed, such as deep belief networks (DBN), auto encoders, long-short term memory (LSTM) and  convolutional neural networks (ConvNets)~\cite{goodfellow2016deep}. 

\begin{figure*}[t]
 \centering
 \includegraphics[width=1\linewidth]{assets/architecture.pdf}
 \caption{Basic frequency layer architecture for image classification.}
 \label{fig:architecture}
\end{figure*}

%convnet intro
%ConvNets are achieving excellent results in the field of computer vision, mainly after 2012\cite{krizhevsky2012imagenet}.

They are inspired on the structure of the visual cortex of the human brain, responsible to process visual information captured by the eye. Each layer in a ConvNet executes a simple operation, such as weighted linear sum of inputs and nonlinear functions such as thresholds, but when several of these layers are arranged in a deep architecture, the network can perform a highly complex and nonlinear transformation of the input data \cite{goodfellow2016deep}.

%One of the main benefits of ConvNets is that they worked directly in the raw data, learning directly from the image pixels in the case of a computer vision application. In this sense, it is not necessary a high domain knowledge of a human specialist to design a feature extractor as described earlier\cite{haykin2009neural}. 

%In order to allow to create these architectures, four main concepts are employed in ConvNets: local connections, shared weights, grouping or pooling and the use of multiple layers \cite{lecun2015deep}. 

Four main concepts are explored in ConvNets: local connections, weight sharing, pooling and the use of stacked layers \cite{lecun2015deep}. 
Basically, when used for image classification, the network process the input pixels in different layers, performing convolution operations using shared convolution weights and extracting features from local connections. These features are then activated by a non-linear function and grouped. The output of these operations is then used as input for to the next layer until achieves the last one, which will generate the probability for each class as the output.

Nowadays due to its excellent performance, ConvNets are being applied in many real life applications, such as autonomous vehicles, object detection and recognition and image labeling \cite{lecun2015deep}.

%One interesting thing is that convolution functions can be performed as a multiplication in the frequency domain\cite{gonzalez2003digital}. This opens a new perspective for research exploring the frequency components, which may be very useful to solve many problems. This paper goes in this direction, presenting a way of use the frequency domain effectively for image classification problems.

From the theory of Fourier transform, it is well-known that a convolution in the space domain becomes a multiplication in the frequency domain. So, it is perfectly possible to process the available data by working in the frequency domain, instead of performing the spatial convolution. 

This fact raises an intriguing question: what if a neural network was entirely designed to operate in the frequency domain? It is important to bear in mind that it is not referring to a standard ANN whose inputs are features in the frequency-domain representation. Rather, in this learning model the operations will be, in fact, adapted to the frequency domain, in light of the theory of Fourier transform. 

In this context, other important questions naturally arise, such as: what would be the model of a frequency-domain layer? How efficiently train such layers? Is it possible to extract both global and local frequency-domain information from the input data? And, finally, what are the advantages of explicitly exploring the frequency domain, instead of using the well-established ConvNets?

The motivation for such a model comes from the idea that, depending on the problem, useful properties of the input data for the task at hand can be more easily perceived and extracted in the frequency domain, rather than on its raw pixels. For instance, when classifying different plantations on images captured by a drone, probably the frequency representation will bring more useful information due to the periodical nature of the data. In these images, high frequency components represent fine details, such as plants borders and corners, whereas low frequency components encode large scale information, such as shape and homogeneous areas of the plants and soil. Still, intermediate concentrations of frequencies in certain 2D spectrum regions will represent the periodical spacing between plants in such agriculture.

It is important to say that Fourier analysis is widely applied in conjunction with ANNs for decades, in different applications, such as brain electroencephalogram processing~\cite{srinivasan2005artificial}, cardiovascular analysis\cite{malliani1991cardiovascular}, speech processing\cite{wang2015speech}, seismic analysis~\cite{dowla1990seismic} and face spoofing detection\cite{stuchi_mlsp}. There are applications on deep learning as well such the ones in the speech processing field~\cite{graves2013speech, silva2017exploring}, where an audio signal is converted into a 2D spectrogram image. 

However, this work is different since it is not using features handcrafted extracted from the frequency domain, but it allows the network to learn the filters that boost the most discriminative components for that specific classification problem.

In this sense, the present work addresses all the aforementioned questions and presents a new neural network model that explores frequency-domain layers and can be applied to different computer vision problems. The proposed model, named FreqNet, is characterized by layers of frequency filters, which extract features from the magnitude spectrum of the image, and whose parameters are adjusted with the aid of gradient-based optimization methods using the error backpropagation algorithm. 

%By training the coefficients of the frequency filters, the FreqNet learns to emphasize the most discriminative frequency components of the data. 



%Depending on the problem, the frequency domain can bring more useful information, providing easily detected features in the image spectrum rather than in the raw pixels. While high frequency components represent both fine details (\textit{e.g., soft borders}) and noise, low frequency components encode large scale information, such as shape and homogeneous areas~\cite{gonzalez2003digital}.

%In this scenario, Fourier analysis is widely applied. In many application it is used in conjunction with neural networks such as brain electroencephalogram processing~\cite{srinivasan2005artificial}, cardiovascular analysis\cite{malliani1991cardiovascular}, speech processing\cite{wang2015speech}, seismic analysis~\cite{dowla1990seismic} and face spoofing detection\cite{stuchi_mlsp}.

%The main application using deep learning and the Fourier spectrum is related to speech processing~\cite{graves2013speech, silva2017exploring}, where an audio signal is converted into a 2D spectrogram image. 
%ADD MORE FREQUENCY DOMAIN + DNN HERE

%In this scenario, this paper presents a new way of training neural networks in the frequency domain in order to be applied in image classification problems. This method is generic and can be applied to different computer vision problems, extracting information directly from the domain spectrum by training frequency filters weights, which boost the more distinguishable components. 

The current work is an extension of the paper presented by the authors in \cite{stuchi_mlsp}, now presenting a technique to train the frequency domain filters. In the previous paper, fixed frequency domain filters were used in conjunction with the idea of slicing the image in blocks in order to capture global and local frequencies components. In the current proposal, the frequency filters for each block are trained using the back-propagation algorithm, allowing the proposed network to achieve excellent results, comparable to the ones obtained by ConvNets.

%Textures and retina images were used to evaluate the proposed method performance. They are also compared with deep learning architectures in order to understand the real contribution when compared with state-of-the-art methods. 

The next sections will present the research and results achieved in this sense and they are organized as follows. Section 2 describes the basic architecture proposed and the method used to train the network on the frequency domain. Section 3 brings some experiments performed in different datasets, like texture and retina images, in order to evaluate the method. In this section the results and comparison with deep learning architectures are also presented in order to understand the real contribution of the proposed method. Finally, Section 4 presents the conclusion and perspective for future research and applications.



